STAR: A Foundation Model-driven Framework for Robust Task Planning and Failure Recovery in Robotic Systems

Modern robotic systems, deployed across domains from industrial automation to domestic assistance, face a critical challenge: executing tasks with precision and adaptability in dynamic, unpredictable environments. To address this, we propose STAR (Smart Task Adaptation and Recovery), a novel framework that synergizes Foundation Models (FMs) with dynamically expanding Knowledge Graphs (KGs) to enable resilient task planning and autonomous failure recovery. While FMs offer remarkable generalization and contextual reasoning, their limitations, including computational inefficiency, hallucinations, and output inconsistencies hinder reliable deployment. STAR mitigates these issues by embedding learned knowledge into structured, reusable KGs, which streamline information retrieval, reduce redundant FM computations, and provide precise, scenario-specific insights. The framework leverages FM-driven reasoning to diagnose failures, generate context-aware recovery strategies, and execute corrective actions without human intervention or system restarts. Unlike conventional approaches that rely on rigid protocols, STAR dynamically expands its KG with experiential knowledge, ensuring continuous adaptation to novel scenarios. To evaluate the effectiveness of this approach, we developed a comprehensive dataset that includes various robotic tasks and failure scenarios. Through extensive experimentation, STAR demonstrated an 86% task planning accuracy and 78% recovery success rate, showing significant improvements over baseline methods. The framework's ability to continuously learn from experience while maintaining structured knowledge representation makes it particularly suitable for long-term deployment in real-world applications.

==> 3-foon.tex <==
\section{Background}

\subsection{Functional Object-Oriented Network}
\label{sec:FOON}
% \subsection{Basics of FOON}
A FOON is a bipartite network with two types of nodes: \textit{object nodes} and \textit{motion nodes}.
Affordances~\cite{Gibson_1977} are depicted via edges that connect objects to actions and enforce action sequencing.
A fundamental structure known as a \textit{functional unit} represents actions in FOON by describing the state change of objects before and after execution, and it has \textit{input} object nodes, \textit{output} object nodes, and a motion node.
% , where states can be used to determine when an action has been completed~\cite{jelodar2018identifying,jelodar2019joint}.
% collection of object and motion nodes to describe a single action within an activity called .
% The coupling of object and motion nodes to represent a single action is referred to as a \textit{functional unit}.
% {\color{red}[C-2.2] 
% {\it Input} object nodes describe the required state(s) of objects for an action, and {\it output} object nodes describe the outcome of executing said action.
% % }
% {\it Input} and  {\it output} nodes describe the required state(s) of objects for an action, and the outcome of execution respectively.
% % }
It is akin to a planning operator in PDDL (short for \textit{Planning Domain Definition Language})
~\cite{mcdermott1998pddl}, where input and output nodes describe preconditions and effects respectively.
Figure~\ref{fig:unit} depicts examples of functional units for the action sequence of: 1) picking and placing a \textit{whole tomato} on a \textit{cutting board}, 2) slicing the \textit{tomato} with a \textit{knife}, and 3) pouring the \textit{sliced tomato} from the \textit{cutting board} into a \textit{bowl}.

Typically, we create FOONs by annotating video demonstrations.
A FOON representing a single activity is referred to as a \textit{subgraph}; a subgraph contains functional units in sequence to describe objects' states before and after each action occurs, and what objects are being manipulated.
Presently, this annotation process is done manually, but previous work has investigated how graphs can be annotated in a semi-automatic manner~\cite{jelodar2018long}.
Two or more subgraphs can be merged together to form what we call a {\it universal FOON}. 
A universal FOON can contain variations of recipes once it has been merged with several sources of knowledge. 
This merging procedure is simply a union operation applied to all functional units from each subgraph we wish to combine; as a result, duplicate functional units are eliminated in the merged network~\cite{paulius2016functional}.
Presently, FOON comprises of 140 subgraph annotations of videos from YouTube, Activity-Net~\cite{caba2015activitynet}, and EPIC-KITCHENS~\cite{Damen2018EPICKITCHENS}, which are all available on our website~\cite{foonet}.

\begin{figure}[!t]
	\centering
    \includegraphics[width=0.9\columnwidth]{figures/fig-FOON-140-4.pdf}
	\caption{
	Illustration of a universal FOON made of 140 recipe subgraphs, and three (3) connected functional units, where object nodes are denoted by green circles and motion nodes are denoted by red squares.
% 	The functional units describe the action sequence of: picking-and-placing a \textit{whole tomato} on a \textit{cutting board}, slicing the \textit{whole tomato} using a \textit{knife}, and pouring the \textit{sliced tomato} into a \textit{bowl}.
	}
	\label{fig:unit}
	\vspace{-0.2in}
\end{figure}




%%%%%%%%%%%%%% commented to compress to maintain page limit %%%%%%%%%%%%%%
% \subsection{Definitions}
% %%%%% From ICRA 2022 submission:
% % A typical FOON graph has two types of nodes, \textit{object nodes} and \textit{motion nodes}, which makes it a bipartite network.
% % Affordances~\cite{Gibson_1977} are depicted with edges that connect objects to actions, which also indicate order of actions in the network.
% % To represent actions in FOON, we use a collection of object and motion nodes to describe a single action within an activity called a \textit{functional unit}.
% % A functional unit describes the state change of objects before and after execution, where states can be used to determine when an action has been completed~\cite{jelodar2018identifying,jelodar2019joint}.
% % {\it Input} object nodes describe the required state(s) of objects for an action, and {\it output} object nodes describe the outcome of executing said action.
% % In Figure~\ref{fig:unit}, we show an example of two functional units for: 1) picking-and-placing an onion onto a cutting board, and 2) slicing the onion with a knife.
% % Some actions may not cause a change in all input objects' states, so there may be instances where there are fewer output object nodes than inputs; for instance, in Figure~\ref{fig:unit}, the \textit{onion} object's state changes across each functional unit, while the \textit{knife} object does not change as a result of the slicing action.
% \subsubsection{Functional Object-Oriented Network}
% The \textit{functional object-oriented network} (FOON) is a knowledge graph representation that takes the form of a bipartite graph, which is a graph that contains two types of nodes.
% It captures the essence of manipulation action sequences using its depiction of actions via \textit{object nodes} and \textit{motion nodes}.

% \subsubsection{Object nodes}
% Object nodes are nodes that refer to objects that are either: 1) directly manipulated by a demonstrator, or 2) indirectly manipulated via interaction with other objects.
% To represent cooking activities, these nodes reflect objects such as ingredients (e.g., vegetables, seasonings, condiments), utensils (e.g., knife, spoon, fork), containers (e.g., bowl, cutting board, bottle), and appliances (e.g., stove, oven, microwave).

% Object nodes are identified by an object type and label, its state type (e.g., \textit{whole}, \textit{sliced}, \textit{mixed}, \textit{grated}, \textit{raw}), and its ingredient composition in the case of composite objects or containers (i.e., what ingredients are contained or makes up an object).
% An example of a composite object is a finished meal such as \textit{scrambled eggs}, which would be made up of multiple ingredients like \textit{egg}, \textit{salt}, and \textit{pepper}.

% \subsubsection{Motion nodes}
% Motion nodes are nodes that refer to actions in which objects are interacted in some way either through manipulation (e.g., \textit{picking}, \textit{placing}, \textit{cutting}, \textit{pouring}, \textit{stirring}) or non-manipulation interactions, especially those that rely on perceptual cues (e.g., baking, cooking, boiling).

% \subsubsection{Functional units}
% Object nodes and motion nodes are connected via directed edges, which reflect a sequencing of actions that may or may not change the state of objects.
% A single action with a motion node that causes a transition of object states for incoming edges (known as \textit{input object nodes}) to produce a new set of object nodes (known as \textit{output object nodes}) is referred to as a \textit{functional unit}.
% Object nodes are kept unique throughout a FOON, while motion nodes can be repeated to correspond to variations of functional units.
% Additionally, within the context of a functional unit, objects are assigned \textit{motion identifier flags}, which describe whether an input or output object node are actively manipulated (i.e., moved directly by a gripper or hand) or not (i.e., an object moves because of another active object, or no motion is observed) with values of 1 and 0 respectively.
% This can be useful to determine the main object from which we observe a trajectory.

% A functional unit can be likened to a planning operator in the PDDL planning language~\cite{mcdermott1998pddl}, where input object nodes correspond to preconditions and output object nodes correspond to effects.
% Some actions may not cause a change in all input objects' states, so there may be instances where there are fewer output object nodes than input object nodes.
% The resulting states of the output objects are necessary for determining whether a functional unit has been fully executed or not~\cite{jelodar2018identifying,jelodar2019joint}.

% We illustrate an example of functional units in Figure~\ref{fig:unit}, which depicts three (3) functional units that correspond to the actions of picking-and-placing a \textit{whole tomato} on a \textit{cutting board}, slicing the \textit{whole tomato} using a \textit{knife}, and pouring the \textit{sliced tomato} from the \textit{cutting board} into a \textit{bowl}.
% In this case, objects such as the \textit{knife} does not undergo a state change and thus does not appear as an output object node.

% %%%%%%%% commented to follow the author guideline %%%%%%%%

% \begin{figure}[t]
% 	\centering
%     \includegraphics[width=\columnwidth]{figures/1-FOON-140.pdf}
% 	\caption{Illustration of: \textbf{(A)} a universal FOON made of 140 recipe subgraphs, and \textbf{(B)} three (3) connected functional units, where object nodes are denoted by green circles and motion nodes are denoted by red squares. The functional units in \textbf{(B)} describe the action sequence of: picking-and-placing a \textit{whole tomato} on a \textit{cutting board}, slicing the \textit{whole tomato} using a \textit{knife}, and pouring the \textit{sliced tomato} into a \textit{bowl}.
% 	}
% 	\label{fig:unit}
% \end{figure}
% %%%%%%%%%%%%

% %%%%% From ICRA 2022 submission:
% % A FOON is created by annotating video demonstrations into the FOON graph structure.
% % A FOON that represents a single activity is referred to as a {\it subgraph}; a subgraph contains functional units in sequence to describe objects' states before and after each action occurs,  and what objects are being manipulated.
% % Presently, annotation is done manually, but efforts have been made to investigate how we can annotate graphs in a semi-automatic procedure~\cite{jelodar2018long}.
% % Two or more subgraphs can be merged together to form what we call a {\it universal FOON}. 
% % A universal FOON could propose variations of recipes once it has been created from merging graphs obtained from several sources of knowledge. 
% % This merging procedure is simply a union operation applied to all functional units from each subgraph we wish to combine; as a result, duplicate functional units are eliminated.
% % Presently, our FOON dataset comprises of 111 subgraph annotations of videos from YouTube, Activity-Net~\cite{caba2015activitynet}, and EPIC-KITCHENS~\cite{Damen2018EPICKITCHENS}, which are all available on our website~\cite{foonet}.

% \subsubsection{Subgraph}
% By using functional units, which are the fundamental learning units of FOON, we are able to vividly describe actions as seen in demonstrations.
% We refer to a sequence of functional units that describes a single activity, recipe, or demonstration as a FOON \textit{subgraph}. 
% Typically, a subgraph is created by an annotator who watches an instructional video and notes observed objects and actions as functional units.
% Presently, our FOON dataset\footnote{FOON dataset -- \url{http://www.foonets.com}} is made up of a total of 140 subgraphs, which correspond to recipe and demonstration videos from YouTube, Activity-Net~\cite{caba2015activitynet}, and EPIC-KITCHENS~\cite{Damen2018EPICKITCHENS}.
% These annotations along with useful starting code to process the files are provided online.

% \subsubsection{Universal FOON}
% Using a collection of two or more subgraphs, we form a comprehensive knowledge graph, which we refer to as a \textit{universal FOON}.
% A universal FOON is created through a merging operation~\cite{paulius2016functional}, which is used to consolidate different ways of making certain ingredients or meals and to find overlapping functional units that may be common across a variety of recipes by identifying duplicate units.
% Duplicate functional units will share the exact combination of input and output object nodes and motion node.

% \subsubsection{Task tree}
% FOON provides an intuitive representation of activities, as it relates to objects, states, manipulations and actions, in the form of a knowledge graph.
% Other than serving as a knowledge representation, a robot can retrieve knowledge from FOON for problem solving, where a problem is defined as a goal (i.e., a target object, such as a finished meal in the case of cooking) that needs to be achieved.
% In terms of FOON, this means finding a sequence of functional units, which would be a subset of a universal FOON, that reaches the target object from an initial state of the environment.
% We refer to this sequence of units as a \textit{task tree}.


% \subsection{Statistics}
% In Figure~\ref{fig:foon_stats}, we report the top 10 most frequently used object (ingredients and utensils), state, and motion labels found in the universal FOON we use in our paper, which is formed from the 140 videos mentioned before.
% %%%%%%%%%%%%%% commented to compress to maintain page limit %%%%%%%%%%%%%%
% % In Figure~\ref{fig:summary}, we compare statistics of the universal FOON with the Recipe1M+~\cite{marin2019learning} dataset, which we use in our experiments. We also illustrate the distribution of recipes by dish types, which we require for our task tree generation method. However, Recipe1M+ does not provide the dish class assignments for each recipe; therefore, we inferred that by using the dish class as a keyword in a Recipe1M+ recipe's title (e.g., for \textit{salad} recipes, we search for recipes that contain the word ``salad'' in the title). Since the actions in FOON are organized in a structured way using functional units, it is easy to identify the ingredient with its state, utensil, and applied motion separately. Recipe1M+ recipes consist of a list of required ingredients and their states, but they do not explicitly provide details on the required utensils and manipulation actions.
% %%%%%%%%%%%%%%
% % \begin{figure}[t]
% % 	\centering
% % 	\includegraphics[width=0.9\linewidth]{figures/fig-universal_FOON.pdf}
% % 	\caption{Illustration of a universal FOON made of 140 instructional videos. 
% % 	This network, along with other subgraphs, are available on our website.}
% % 	\label{fig:FOON}
% % \end{figure}


% %%%%%%%% commented to follow the author guideline %%%%%%%%
% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=\columnwidth]{figures/2-stat-FOON.pdf}
% 	\caption{Top 10 most frequently seen \textbf{(A)} motions, \textbf{(B)} ingredients, \textbf{(C)} states and \textbf{(D)} utensils in FOON.}
% 	\label{fig:foon_stats}
% \end{figure}

% %%%%%%%%%%%%%% commented to compress to maintain page limit %%%%%%%%%%%%%%
% % \begin{figure}[t]
% % \begin{center}
% % \includegraphics[width=\columnwidth]{figures/3-comparison-dataset.pdf}
% % \end{center}
% % \caption{Distribution of \textbf{(A)} FOON, \textbf{(B)} Recipe1M+ recipes in 30 dish classes. \textbf{(C)} Comparison of the two datasets in terms of the total number of recipes, ingredients, utensils, states and motions used.}
% % \label{fig:summary}
% % \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%

% %%%%%%%%%%%%%% %%%%%%%%%%%%%% %%%%%%%%%%%%%% %%%%%%%%%%%%%% 
\subsubsection{Task Planning with FOON}
% {\color{red} Some parts of this section are described in introduction. So may be we can compress this. Or, may be we can completely remove this subsection.}
%%%%% From ICRA 2022 submission:
% In addition to representing knowledge, a robot can use FOON for problem solving.
% Through a process of \textit{task tree retrieval}, a robot can obtain a subgraph, known as a \textit{task tree}, that contains the steps (i.e., functional units) it needs to execute to achieve some sort of goal.
% A task tree differs from a regular subgraph, as it may not exactly match  human demonstration; rather, it will leverage knowledge from multiple sources to produce a novel task sequence.
% The conventional retrieval algorithm requires a list of items in its environment to identify ideal functional units based on the availability of inputs to these units~\cite{paulius2016functional}.
% The algorithm draws upon the depth-first search (DFS) and breadth-first search (BFS) algorithms: starting from the goal node, we search for candidate functional units in a depth-wise manner, while for each candidate unit, we search among its input nodes in a breadth-wise manner to determine whether or not they are in the kitchen.
% In~\cite{paulius2021weighted}, we introduced an alternative retrieval algorithm that explores different paths to achieving a goal; this was used to evaluate the most optimal path with a weighted FOON, where each functional unit is assigned a weight corresponding to its success rate of execution.
% This version of the algorithm is used to derive task trees for our task tree generation procedure. A limitation of the previous retrieval approach is that it cannot generate a task tree if the exact recipe does not exist in the graph. For example, it cannot produce the task plan of a ``corn soup" even though it knows about ``potato soup". Also, it cannot infer the task plan for a new ingredient that was never seen before.

Task planning involves retrieving a \textit{task tree}~\cite{paulius2016functional} (a high-level task plan) that satisfies a goal defined as an object node.
Finding a task tree requires knowledge about the state of a robot's environment, specifically what objects are available and the state(s) in which they are in.
% We refer to this list of objects as the \textit{kitchen} list, since it is related to cooking.
% The algorithm works by finding functional units that satisfies all requirements of the goal node in a manner that combines conventional depth-first search (DFS) and breadth-first search (BFS) algorithms: starting from the goal node, we search for candidate functional units in a depth-wise manner, and then, for each candidate unit, we search among its input nodes in a breadth-wise manner.
Starting from the goal, the algorithm searches for candidate functional units in a depth-wise manner, and then, for each candidate unit, it searches its input nodes in a breadth-wise manner to see if they are available to the robot.
%to determine whether or not they are available in the kitchen.
% If certain input nodes are not available in the kitchen, then these nodes are also added as sub-goals that need to be satisfied as well in the searching process.
More recently, we introduced a modified version of the algorithm to find the optimal path to reach a goal node, which is reflected by weights given to each functional unit corresponding to its success rate of execution by a robot~\cite{paulius2021weighted}.
However, these algorithms are not suited to generate task trees for recipes not found in FOON; for this task, we use semantic similarity~\cite{paulius2018functional} while searching to modify task trees as required
for a given problem and ingredient set.
% We will introduce these ideas in the following section.



==> 3-related_work.tex <==
\subsection{Related Works}

% Reflect \cite{liu2023reflect}: users ai2thor simulator. main contribution: bridging the gap between sensor data to LLM input. they summarize sensor input into a text format that can be used as llm prompt. from summary of different frames, they try to create execution summary. LLM tries to find mistake in the summary and outputs how to correct the wrong step. for example: fridge was closed, still robot tried to take stuff from it. to convert vision data to scene graph, they use object detector and the bounding boxed image is used for state detection using CLIP.
% issue: if all subgoals are successful but the final goal is not satisfied, they say that the plan was incorrect and ask LLM to correct it. This is inefficient. We try to reduce plan inaccuracy before it even begins execution. Our two main idea: consolidating task plan and creating local database of successful plans. Another issue of their approach is if they achieve the required state for a subgoal, they say that subgoal is successful and move to the next state. But it is possible that there are failures such as spilling, collision even if the goal is satisfied. They observe the result but do not mointor the progress. So, even if a hazard such as broken glass on the floor happens, they won't be able to detect it and stop there. Another issue is that they only consider a limited number of predefined states for each object. 

% SayCan \cite{saycan} computes two values for each action in the skill library. LLM probability is calculated by the LLM (closeness between the high-level instruction and the skill) and value function is the feasibility of executing the action in that state. This two scores are multiplied to calculated the overall score of an action. The action with highest score is executed. 

% CAPE \cite{raman2023cape} provides the error generated by simulator to LLM as a precondition error. LLM then corrects the plan. 
% confusion: how do they get the error in real world? they are not using multi-modal sensors.

% Tree-Planner \cite{hu2023treeplanner} generate multiple plans for a task. Then it creates a aggregated graph by merging common nodes. At each node, it tries to execute an action. If it fails, it goes to try next option. If all option fails, it goes back to parent and invalidate it. Then it tries the sibling of the parent node and this process go on. The purpose of this process is to reduce token generation. 

% Huang et al. \cite{huang2022language} used few shot prompting to generate task plan. They generate one task step at a time. That step may not be executable by the robot. So, they translate the step to a equivalent action that are in robot's skill set. This translation is done using BERT. In next iteration, the selected action is passed to the prompt to generate next action. The plan is evaluated using two metric: executability and correctness. Executability indicates if the plan has correct grammar and meets precondition. Correctness is evaluated by human checking. They used VirtualHome for their experiment. 

% ViLaIn \cite{shirai2024visionlanguage} creates a problem file from the scene observation and task description. Then, assuming that they have the PDDL domain file, they use symbolic planner to generate the Plan. If the planner returns error, they reprompt LLM to regenerate the problem file. This step is called corrective reprompting. The evaluation does not involve robot. They use a plan validator software to evaluate the problem description. 

% ISR-LLM \cite{zhou2023isrllm} uses few-shot prompting in three stages. First, it creates PDDL domain and problem file from the task description. The example prompt includes some examples of (problem description, domain file, problem file) triplets. Next, a plan is generated from the domain and problem file using LLM. In this phase, the prompt example includes (domain file, problem file, plan). In next phase, the plan is validated using LLM and external validator and the plan is refined based on the validator feedback until an error-free plan is found. The LLM validator again uses few-shot prompting. The prompt includes set of (initial state, goal state, plan, validation result with analysis). Until the validation result says that the plan is correct, this refinement continues. The external validator is basically precondition checking. They have hardcoded the precondition for each action. 

% Parakh et al. \cite{parakh2023lifelong} outputs the task plan in the form of python code. Their main contribution is extending the skill library. If LLM outputs an action that is missing in the library, their method teaches the new skill to robot and reuse that skill in the future tasks. 

% Interactive planning was proposed by Sun et al. \cite{sun2023interactive} to solve partially observable tasks. For example, a robot is asked to throw away the empty cup to the bin but it can not see which cup is empty. This is a partially observable situation. They use LLM to generate a plan that will equip the robot to collect the missing information from the environment. In this case, the plan is to collect the weight of the two cups of the force sensor. Then the LLM evaluator analyzes this information and outputs which cup is empty. Finally, the LLM planner use this info to generate a plan to throw the empty cup. For the experiment, they used tabletop environment on IsaacGym.

% AutoTAMP \cite{chen2024autotamp} focuses on correcting the semantic and syntactic error in the task plan generated by LLM. From the insturction and scene observation, they first generate a plan as an intermediate representation named STL (Signal Temporal Logic) using LLM. This plan is check for Sytactical correctness. After that, they use STL planner for the motion planning. The motion plan is checked for semantic accuracy using LLM. For that, they ask LLM if the STL generated plan and the original instruction aligns. If there is any mistake, they re-prompt LLM.

% Faithful Long-Horizon Task planning (no citation found) mentioned that when there are too many rules and constraints to solve a constraints, it is difficult to remember and follow all of that. Even human struggles with that. So, usually human breaks down the long task into smaller tasks and solve them one by one. Following that, in this work, the authors breaks down the instruction into sub tasks. Then, they solve each sub-task one by one. The goal task, rules, initial plan are said long term memory. The sub task goal, instructions and demonstrations are called short term memory. This paper provides long term goal, short term goal and the state observation into the LLM prompt and generate a plan to solve the subtask. The main contribution is just representating the prompt in a formal way. The experiment was done in VirtualHome.

% Arora et al. \cite{Arora2024AnticipateA} used LLM for task anticipation. Usually, we use LLM to create sub-tasks and then handle one subtask at a time. What they do here is that they combine all sub-task and represent them as PDDL goal in problem file. Then they use PDDL planner to come up with a plan. This way often the plan length is smaller. For example, when the agent is fetching the milk from bridge, it can also bring ingredients for making breakfast. They have showed in their experiment that LLM is very good in this kind of anticipation with just a few in-context example. They have conducted the experiment in VirtualHome. One more interesting thing they have shown is human interruption. Action execution was interrupted by the prompt ``There is an urgent meeting now. Do not prepare breakfast''. In this situation, the agent was able to plan suitable actions and put the vegetables back in their original location because it was no longer necessary to cook a hot breakfast; the agent instead computed action sequences to prepare the laptop and suitable clothes for the meeting.


